FIRE-Bench: Evaluating AI Agents on the Rediscovery of Scientific Insights

Autonomous agents powered by large language models (LLMs) promise to accelerate scientific discovery end-to-end, but rigorously evaluating their capacity for verifiable discovery remains a central challenge. Existing benchmarks face a trade-off: they either heavily rely on LLM-as-judge evaluations of automatically generated research outputs or optimize convenient yet isolated performance metrics that provide coarse proxies for scientific insight. To address this gap, we introduce FIRE-Bench (Full-cycle Insight Rediscovery Evaluation), a benchmark that evaluates agents through the rediscovery of established findings from recent, high-impact machine learning research. Agents are given only a high-level research question extracted from a published, verified study and must autonomously explore ideas, design experiments, implement code, execute their plans, and derive conclusions supported by empirical evidence. We evaluate a range of state-of-the-art agents with frontier LLMs backbones like gpt-5 on FIRE-Bench. Our results show that full-cycle scientific research remains challenging for current agent systems: even the strongest agents achieve limited rediscovery success (<50 F1), exhibit high variance across runs, and display recurring failure modes in experimental design, execution, and evidence-based reasoning. FIRE-Bench provides a rigorous and diagnostic framework for measuring progress toward reliable agent-driven scientific discovery.

==> Tables/motivation.tex <==
\begin{table}[t]
  \centering
  \renewcommand{\arraystretch}{1.1}  % Increase spacing between rows
  \begin{tabular}{L{3cm}*{6}{>{\centering\arraybackslash}p{1.5cm}}}
    \toprule
    \rowcolor{Gray}
    \textbf{Benchmark} \textbf{(pub.~date)} &
    \textbf{Cross-domain tasks} &
    \textbf{Full research workflow} &
    \textbf{Real-paper ground truth} &
    \textbf{LLM-based reasoning eval.} &
    \textbf{Code-exec. tools} &
    \textbf{Iterative reflection} \\
    \midrule
    AgentBench \newline (Aug 2023)            & \xmark & \xmark & \xmark & \xmark & \xmark & \xmark \\
    \rowcolor{Gray!30}
    MLAgentBench \newline (Oct 2023)          & \xmark & \xmark & \xmark & \xmark & \cmark & \cmark \\
    InfiAgent-DABench \newline (Jan 2024)     & \cmark & \xmark & \xmark & \xmark & \cmark & \xmark \\
    \rowcolor{Gray!30}
    DiscoveryBench \newline (Jul 2024)        & \cmark & \xmark & \cmark & \cmark & \cmark & \xmark \\
    DSBench \newline (Sep 2024)               & \cmark & \xmark & \xmark & \xmark & \cmark & \xmark \\
    \rowcolor{Gray!30}
    ScienceAgentBench \newline (Oct 2024)     & \cmark & \xmark & \cmark & \xmark & \cmark & \xmark \\
    RE-Bench \newline (Nov 2024)              & \xmark & \xmark & \xmark & \xmark & \cmark & \cmark \\
    \rowcolor{Gray!30}
    DataSciBench \newline (Feb 2025)          & \cmark & \xmark & \xmark & \cmark & \cmark & \xmark \\
    PaperBench \newline (Apr 2025)            & \xmark & \xmark & \cmark & \cmark & \cmark & \cmark \\
    \rowcolor{Gray!30}
    MLRC-Bench \newline (Apr 2025)            & \xmark & \cmark & \xmark & \xmark & \cmark & \cmark \\
    \midrule
    \rowcolor{Gray!10}
    \textbf{ResearchAgentBench}    & \textbf{\cmark} & \textbf{\cmark} & \textbf{\cmark} & \textbf{\cmark} & \textbf{\cmark} & \textbf{\cmark} \\
    \bottomrule
  \end{tabular}
  \vspace{2pt}
  \caption{Key dimensions of prior benchmarks compared with \textbf{RA-Bench}. No existing benchmark satisfies all dimensions simultaneously.}
  \label{tab:ra_bench_comparison}
\end{table}
